Long-Horizon Multi-Robot Rearrangement Planning for Construction Assembly

Robotic assembly planning enables architects to explicitly account for the assembly process during the design phase, and enables efficient building methods that profit from the robots' different capabilities. Previous work has addressed planning of robot assembly sequences and identifying the feasibility of architectural designs. This paper extends previous work by enabling planning with large, heterogeneous teams of robots. We present a planning system which enables parallelization of complex task and motion planning problems by iteratively solving smaller subproblems. Combining optimization methods to solve for manipulation constraints with a sampling-based bi-directional space-time path planner enables us to plan cooperative multi-robot manipulation with unknown arrival-times. Thus, our solver allows for completing subproblems and tasks with differing timescales and synchronizes them effectively. We demonstrate the approach on multiple case-studies to show the robustness over long planning horizons and scalability to many objects and agents of our algorithm. Finally, we also demonstrate the execution of the computed plans on two robot arms to showcase the feasibility in the real world.

==> preamble/espcolors.tex <==
\usepackage{xcolor}
\definecolor{espblack}{RGB}{0,0,0}
\definecolor{espwhite}{RGB}{255,255,255}
\definecolor{espgray}{RGB}{206,206,206}
\definecolor{esplightgray}{RGB}{224,224,224}
\definecolor{espdarkgray}{RGB}{168,168,168}
\definecolor{espsomewhatdarkgray}{RGB}{130,130,130}
\definecolor{espverydarkgray}{RGB}{100,100,100}
\definecolor{espblue}{RGB}{11,93,174}
\definecolor{esplightblue}{RGB}{59,175,236}
\definecolor{espdarkblue}{RGB}{6,26,64}
\definecolor{espred}{RGB}{206,62,21}
\definecolor{esplightred}{RGB}{206,62,21}
\definecolor{espdarkred}{RGB}{61,19,8}
\definecolor{espyellow}{RGB}{232,163,26}
\definecolor{espgreen}{RGB}{100,161,27}
\definecolor{esplightgreen}{RGB}{149,198,35}
\definecolor{espdarkgreen}{RGB}{49,92,43}
\definecolor{esppurple}{RGB}{106,20,125}
\definecolor{esplightpurple}{RGB}{197,137,232}
\definecolor{espdarkpurple}{RGB}{50,14,59}

==> preamble/mpstikz.tex <==
% PGF/TikZ is a pair of languages for producing vector graphics from geometric/algebraic descriptions.
\usepackage{tikz}

% Tikzscale let's us scale tikzpictures to absolute sizes (e.g., \textwidth) without scaling fonts.
\usepackage{tikzscale}

% PGFPlots provides a friendly and well documented interface for creating plots.
\usepackage{pgfplots}

% PGFPlotsTable provides a friendly and well documented interface for creating tables.
\usepackage{pgfplotstable}

% The calc library enables calculating coordinates, e.g.,
%   \node at ($(0, 1) + (1, 0)$) {hello handsome};
\usetikzlibrary{calc}

% The positioning library allows relative positioning of nodes, e.g.,
%   \node (A) at (0, 0) {handsome};
%   \node [above left = 1pt and 1pt of A] {hello};
\usetikzlibrary{positioning}

% The statistics library adds more plot types to PGF, such as boxplots.
\usepgfplotslibrary{statistics}

% The fillbetween library enables filling the area between curves with color.
\usepgfplotslibrary{fillbetween}

% Define some preset styles for plots.
\pgfplotsset{
  compat=1.15,
  mps basic/.style={
    xlabel near ticks,
    xlabel style={font=\footnotesize},
    ylabel near ticks,
    ylabel style={font=\tiny},
    xmajorgrids,
    major x grid style={dotted},
    ymajorgrids,
    major y grid style={dotted},
    tick label style={font=\tiny}
  },
  mps scientific x/.style={
    x tick label style={
      /pgf/number format/sci,
      font=\tiny
    }
  },
  mps scientific y/.style={
    y tick label style={
      /pgf/number format/sci,
      font=\tiny
    }
  },
  mps fixed x/.style={
    x tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=6,
      /tikz/.cd,
      font=\tiny
    }
  },
  mps fixed y/.style={
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=6,
      /tikz/.cd,
      font=\tiny
    }
  },
  /pgfplots/myylabel absolute/.style={%
      /pgfplots/every axis y label/.style={at={(0,0.5)},xshift=#1,rotate=90,align=center},
      /pgfplots/every y tick scale label/.style={
        at={(0,1)},above right,inner sep=0pt,yshift=0.3em
      }
   }
}

==> preamble/tikz.tex <==
\usetikzlibrary{decorations.pathreplacing,shapes.misc}
\tikzset{
  cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
  cross/.default={4pt},
  start/.style={draw = black, fill = black, circle, inner sep = 0pt, minimum size=3pt},
  goal/.style={draw = black, fill = white, circle, inner sep = 0pt, minimum size=3pt},
  vertex/.style={draw = black, fill = black, circle, inner sep = 0pt, minimum size=0.4pt},
  rgg edge/.style={densely dotted, very thin, espblack},
  forward edge/.style={espblack, thin},
  reverse edge/.style={espgray, thin},
  invalid edge/.style={espblack, thick, densely dotted},
  obstacle/.style={fill = espblack, draw = espblack},
  antiobstacle/.style={draw = none, fill = white},
  boundary/.style={draw = black, fill = none},
  start_region/.style={draw = esplightgreen, ultra thick, fill = none},
  goal_region/.style={draw = espred, ultra thick, fill = none},
  solution/.style={espyellow, very thick}
}

\newcommand{\tikzinlinestart}{\,\protect\tikz[baseline]{\protect\node[start, yshift = 0.25em] {};}\,}
\newcommand{\tikzinlinegoal}{\,\protect\tikz[baseline]{\protect\node[goal, yshift = 0.25em] {};}\,}
\newcommand{\tikzinlinestate}{\,\protect\tikz[baseline]{\protect\node[vertex, yshift = 0.25em] {};}\,}
\newcommand{\tikzinlineobstacle}{\,\protect\tikz[baseline]{\protect\draw[obstacle, yshift = -0.15em] (0,0) rectangle (0.4em, 0.8em);}\,}
\newcommand{\tikzinlinerggedge}{\,\protect\tikz[baseline]{\protect\draw[rgg edge, yshift = 0.25em] (0,0) -- (1.1em, 0);}\,}
\newcommand{\tikzinlinereverseedge}{\,\protect\tikz[baseline]{\protect\draw[reverse edge, yshift = 0.25em] (0,0) -- (1.1em, 0);}\,}
\newcommand{\tikzinlineforwardedge}{\,\protect\tikz[baseline]{\protect\draw[forward edge, yshift = 0.25em] (0,0) -- (1.1em, 0);}\,}
\newcommand{\tikzinlinesolution}{\,\protect\tikz[baseline]{\protect\draw[solution, yshift = 0.25em] (0,0) -- (1.1em, 0);}\,}
\newcommand{\tikzinlinecollision}{\,\protect\tikz[baseline]{\protect\node [cross=4pt, espred, very thick, solid, yshift = 0.3em] {};}\,}

\newcommand{\successplotheight}{0.45\textwidth}
\newcommand{\costplotheight}{0.55\textwidth}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> src/depr.tex <==
\subsection{Discussion \& Limitations}
We discuss some of the limitations of the approach presented here:
\begin{itemize}
    \item The problems we are targeting with this work are highly separable  on  the logical  level,  and  rely  on  needing little interaction, i.e. the subsets of robots we plan for should be small compared to all robots.
    \item The approach to scheduling we propose here is greedy and does not use all the available information, and thus might return suboptimal solutions.
    Clearly, it is possible to approximate e.g. the needed time for the required motions in an action sequence.
    \item The heuristic we use in this work is not optimal, since it is not looking ahead, and exploiting the fact that the evaluation of $\phi$ is usually much cheaper, and taking e.g. statics into account - the limiting factor.
    While the backtracking approach allows us to find solutions to even complex constraint-combinations, in long-horizon construction planning, this is suboptimal.
    Approaches such as backwards assembly planning might be of use to tackle this issue, and inform the forward search from a backwards search \cite{lee92, Kao2017}.
    \item \Cref{tab:comp_time_breakdown} shows that the largest part of the computation time can be attributed to the keyframes generation. Incorporating a more efficient keyframes generator, such as e.g. the one presented in \cite{deharo2020learning} could potentially reduce the necessary computation time, and thus allow us to scale even more.
\end{itemize}
And some limitations regarding the path planning we used in this work:
\begin{itemize}
    \item The problems we tackled here are highly separable, allowing to plan for a large team of robots by focusing on one, or two at a time. In case a problem is more involved, path planning in the joint robot configuration space might not work anymore.
    \item We plan the paths between the mode-switches in a sequential manner.
    While this works very well in the examples we show here, it can be the case that a later transition is more constrained, and thus, it might make more sense to attempt to find a path there first. 
    \item The path planing approach introduced here does not return a time-optimal path.
    Clearly, one could run this in an RRT$^*$-like manner \cite{Karaman2011}.
\end{itemize}




\marc{OLD VERSION BEGIN---}

Due to the non-monotonic nature of the assembly tasks we consider, the order in which objects have to be rearranged (in particular being placed) is not obvious.

A heuristic (which is explained in \cref{sec:tree}) selects a single new object $o_l$ from $\bar{\mathcal{O}}^{l-1}$ and a subset $R_l \subset \mathcal{R}$ of robots that should be involved in rearranging $o_l$ to its target pose $p_{o_l}^G$.



Due to the non-monotonic nature of the assembly tasks we consider, the order in which objects have to be rearranged (in particular being placed) is not obvious.
For example, objects need sufficient support in order to be placed, while placing some objects too early might obstruct later placements.
Let us explicitly express such object-order-constraints as $\phi(O_l; \mathcal{O}^{l-1})\le 0$.

%We begin by formulating the approach for deciding the order in which pieces need to be placed in an empty environment to build up the final model.
%Generally, the set of all possible discrete state sequences $\mathbb{S}(\mathcal{S}, O_{1:n})$ to place all objects is represented as a tree which is induced by the first-order logic rules.

%Therefore, deciding on an object $O_l$ and the robots 

%the object $O_l$ is represented as part of a tree which is induced by the first-order logic rules.
%Therefore, solving \eqref{eq:our_rearrangement} requires tree search

%We call the tuple $v^l = (O_l, R_l, \left\{s_{r, K_r^{l-1}:K^l_r}\right\}_{r\in R_l})$ of the object $O_l$, the set of robots that are involved in placing the object, and their associated discrete state sequence 

%Similar to~\cite{Garrett2020RSS, Krontiris2015}, we define the state space over which we search a possible order of parts:

We begin by formulating the approach for deciding the order in which pieces need to be placed in an empty environment to build up the final model.
The \marc{state as an element of a tuple???} state $v^l\in (O_l, R_l, s_{R, K_r^{l-1}:K^l_r})$ is a tuple of an object $O_l$, the subset of robots that is used to place the object, and the state sequence $s_i$ which is used to place the object, and thus fully defines \textit{one} receding horizon subproblem.
While the discrete state sequence implicitly describes the object, and the robots that are being used in step $l$, we represent them explicitly in $v^l$.
Thus, deciding on an order of objects can be formalized as tree search over the $v^l$.
Hence, we need to find a path from $v^0 = \{\}$ to $v^G$, where $v^G$ is any node where all the objects have been placed successfully.

%In practice, we obtain $s_{R, 1:K^l_r}$ using a logic language and tree-search, see e.g. [cite PDDL/LGP?]. 

\subsubsection{Tree expansion}
A node $v^l$ is \textit{feasible} if there exists a valid solution to \eqref{eq:our_rearrangement}.
Ideally, one would solve \eqref{eq:rearrangement} to obtain the optimal assignment of all actions and objects to robots.
However, this is not possible.

In practice, the heuristic to use for expansion of the tree depends on the cost function $c(\cdot)$.
In the following, we assume $c=1$, since we want to minimize the \textit{make-span}, i.e. the total needed time until all objects are placed at their respective goal locations.

Thus, we introduce a greedy scheduler:
%

%
where $h(O_i; \mathcal{O}^{l-1})$ describes some cost function that solely depends on the placed objects, $V_A(v^l)$ denotes the set of nodes we unsuccessfully attempted in the current state $v^l$.
While we choose $\max_{r\in R} T^l_{r_j}$ as our metric in the greedy scheduler, it is also possible to use, e.g., the sum of all times, or the average time needed.
However, obtaining $T^l_{r_j}$, i.e. the time at which a robot $r_i$ is done with its actions is not possible without actually computing the plan for the robot.
Since computing this is expensive, we approximate it by choosing the \textit{earliest available} agents.
It would also be possible to approximate \eqref{eq:greedy} by estimating the necessary time via e.g. straight-line distance.
In addition, in case the robots have largely the same capabilities, it is possible to decouple choosing $O_l$ via the minimization of $h$, and the action sequence $S_i$:
%
\begin{align}\label{eq:priorization_approximation}
    S_l = \arg &\min_{\substack{R\subseteq \mathcal{R} \\ S\in\mathbb{S}_{R}(\mathcal{S}_{R}, O_l)}} \max_{r\in R} T^{l-1}_{r}\notag\\
    \text{s.t.}~~~& (O_l, R, S)\notin V_A(v^l)
\end{align}
%
We note that this approach can easily be extended to plan the placement of multiple pieces at once, as e.g. proposed in \cite{Hartmann2020} -- this could lead to sequences that are more easily satisfying $\phi$, and might even be necessary for some specific assemblies, where intermediate stability is important.

\subsubsection{Multi-Bound-Tree-Search}\vh{maybe also get rid of this - this is not referred to anywhere else (in the code it happens implicitly, since we do not plan at all, if no feasible keyframes can be found)}
Since fully planning a path for an object placement is computationally expensive, it is desirable to quickly determine feasibility of a node by evaluating a simpler problem.
To achieve this, a lower bound for feasibility is computed as presented in \cite{17-toussaint-ICRA}.
In our setting, possible lower bounds are e.g. attempting to find a possible placement-, or handover-pose for a given object and a robot: If this can not be solved, clearly no solution to the full problem can be found.

Note that such lower bounds can be used for forward-checking of sequences - we do not do this here.

% \subsubsection{Deferred Evaluation}\vh{get rid of this?}
% As in both \cite{Garrett2020RSS, Hartmann2020}, we adopt the deferred evaluation of nodes, i.e., we do only evaluate possible nodes once they are being expanded, thus saving computation time.
% A node being evaluated means that we attempt to find a way to place a part with the given action sequence, which is computationally expensive.

\subsubsection{Backtracking}
If the attempted placement of an object is infeasible, the sequence that was used will be added to $V_A$.
In case no feasible sequence can be found in $n_\text{max}$ attempts, we start backtracking to the previous nodes, and attempt to find a sequence to successfully place the object $O_l$ that lead to a dead end in the tree-search.
%We show an exemplary exploration sequence in \cref{fig:ex_graph}.

In general, the methods we use for generating motion paths for the robots can not prove infeasibility of a specific sequence.
Hence, we keep a list of all leaf nodes that we determined to be infeasible before, and deprioritize the expansion of these nodes.
This allows us to expand more promising states, while still guaranteeing that a solution will be found eventually.

%\cref{fig:ex_schedule}.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.6\linewidth]{img/graph_reasoning.png} 
%     \caption{An exemplary exploration sequence, necessitating backtracking due to the infeasibility of placing $p_3$ after $p_2$.\vh{make nicer}}
%     \label{fig:ex_graph}
% \end{figure}

\marc{---OLD VERSION END}









\subsection{Logic Geometric Programming for Multi Robot Rearrangement Planning}
Given a scene of $n$ unique objects $O_{i}\in\mathcal{O}$, $i=1,\ldots, n$, with their initial poses $p_i^0\in SE(3)$ at time $t = 0$, and $m$ robots $r_{1:m}$, the aim is to \emph{rearrange} all objects to their (given) goal locations $p_i^G\in SE(3)$.
Each robot may have its own configuration space $\mathcal{Q}_i\subset\mathbb{R}^{m_{q_i}}$, i.e.\ we do not restrict our framework to homogeneous robot teams.
We formalize the rearrangement planning problem within the framework of Logic Geometric Programming (LGP).

The idea behind LGP is the formulation of an optimization problem over the continuous path $x: [0,T]\rightarrow\mathcal{X}=\mathcal{Q}\times SE(3)^n$ of all robots ($\mathcal{Q} = \mathcal{Q}_1\times \cdots \times \mathcal{Q}_m$) and objects ($SE(3)^n$), where the constraints at different phases of the motion are determined by a discrete variable $a$, which represents the state of a logic domain.
The standard LGP formulation represents $a$ as a sequence of symbolic states that is determined by a sequence of grounded actions.
Here, we reformulate the notion of $a:[0,T]\rightarrow\mathcal{A}$ to be function of continuous time $t$ that maps into grounded states of the logic domain $\mathcal{A} = \mathcal{A}_1\times \cdots \times \mathcal{A}_m$.

Therefore, our LGP formulation tries to find the time $T>0$, the function $a$, and the path $x$ to optimize
%
\begin{subequations}\label{eq:rearrangement}
\begin{align} 
    \min_{\substack{T,~x:[0,T]\rightarrow\mathcal{X},\\ a:[0,T]\rightarrow \mathcal{A}}} ~&\int^T_0 c(\ddot x(t), \dot x(t), x(t))\diff t \\
    \text{s.t.}~~~~~~~ & x(0) = x_0\big(p_{1:n}^0\big) \\
    \forall t\in[0,T]:~\ & g(x(t), \dot x(t), a(t)) \leq 0 \label{eq:rearrangement:constraint}\\
    & a \in \mathbb{A}(r_{1:m}, O_{1:n}) \label{eq:rearrangement:logic}\\
    & g_\text{goal}\left(x(T), p^G_{1:n}, O_{1:n}\right)\leq 0.  \label{eq:rearrangement:goal}
\end{align}
\end{subequations}
%
%Here, $x$ maps time into the configuration space $\mathcal{Q} = \mathcal{Q}_1\times \cdots \times \mathcal{Q}_m$ of all robots and objects $SE(3)^n$.
%
When evaluated at a time $t$, $a(t)\in\mathcal{A}$ is a vector whose components $a_i(t) \in\mathcal{A}_i$ specify for each robot $i$ the currently active constraints via the function \eqref{eq:rearrangement:constraint}.
For example, $a_i(t_1)$ could specify the necessary constraints for the robot $i$ that it grasps an object at time $t_1$.
Refer to \cref{fig:schedule} for a visualization of an $a$.
\vh{TODO}
%We show an example for $a$ with x robots in \cref{fig:schedule}. 
The set $\mathbb{A}(r_{1:m}, O_{1:n})$ is the space of all valid functions $a$ induced by a first order logic language for the robots $r_{1:m}$ and objects $O_{1:n}$.
The goal constraint \eqref{eq:rearrangement:goal} specifies that at the end of the path ($t=T$) all objects have to be at their target poses.
The initial condition $x_0\big(p_{1:n}^0\big)$ contains the initial configuration of all robots as well as the initial poses of the objects.
Finally, $c$ is a cost function, such as path length, control costs or minimal time.






% \begin{subequations}
% \begin{align} \label{eq:our_rearrangement}
%     \min_{\substack{T^k_i,~x^k(\cdot),~a^k(\cdot)}} ~&\int^{T^k_i}_{T_i^{k-1}} c(\ddot x(t), \dot x(t), x(t))\diff t \\
%     \text{s.t.}~~~~~~~ & x^k(t) = \left[x^k_\text{p}(t), x^k_\text{np}(t)_{r_i}, x^k_\text{np}(t)_{O_i} \right]\\
%     & a^k(t) = \left[a^k_\text{p}(t), a_\text{np}(t)_{r_i} \right]\\
%     \forall t\in[T_i^{k-1},T_i^{k}]:~\ & g(x(t), \dot x(t), a(t)) \leq 0\\
%     & a \in \mathbb{A}(r_{1:m}, O_{1:n}) \label{eq:our_rearrangement:logic}\\
%     & g_\text{goal}\left(x(T_i^k), p^G_i, O_i\right)\leq 0.  \label{eq:our_rearrangement:goal}
% \end{align}
% \end{subequations}

%\begin{subequations}
%\begin{align} \label{eq:our_rearrangement}
%    \min_{\substack{T^k_i,~x_{r_i, O_i}:\left[T_i^{k-1},T_i^k\right]\rightarrow\mathcal{X}_{r_i, O_i},\\ a_{r_i}:\left[T_i^{k-1},T_i^k\right]\rightarrow \mathcal{A}_{r_i, O_i}}} ~&\int^{T^k_i}_{T_i^{k-1}} c(\ddot x(t), \dot x(t), x(t))\diff t \\
%    \text{s.t.}~~~~~~~ & x^k(t) = \left[x^k_\text{p}(t), x^k_{r_i, O_i}(t) \right]\\
%    & a(t) = \left[a_i^\ast(t), a_{r_i}(t) \right]\\
%    \forall t\in[0,T_i]:~\ & g(x(t), \dot x(t), a(t)) \leq 0\\
%    & a_{r_i} \in \mathbb{A}_{r_i}(r_{1:m}, O_{1:n}) \label{eq:our_rearrangement:logic}\\
%    & g_\text{goal}\left(x_{O_i}(T_i), p^G_i, O_i\right)\leq 0.  \label{eq:our_rearrangement:goal}
%\end{align}
%\end{subequations}
















%Dantam 2018 \cite{Dantam2018} (Constraint-based TAMP)

%Dogar 2019 \cite{Dogar2019} (Collaborative assembly using regrasp operations inbetween actions. Solves a subproblem which we do not consider. Their work is thus complementary.)

